Domain Adaptation for Named Entity Recognition in Online Media with Word Embeddings

Content on the Internet is heterogeneous and arises from various domains like News, Entertainment, Finance and Technology. Understanding such content requires identifying named entities (persons, places and organizations) as one of the key steps. Traditionally Named Entity Recognition (NER) systems have been built using available annotated datasets (like CoNLL, MUC) and demonstrate excellent performance. However, these models fail to generalize onto other domains like Sports and Finance where conventions and language use can differ significantly. Furthermore, several domains do not have large amounts of annotated labeled data for training robust Named Entity Recognition models. A key step towards this challenge is to adapt models learned on domains where large amounts of annotated training data are available to domains with scarce annotated data. In this paper, we propose methods to effectively adapt models learned on one domain onto other domains using distributed word representations. First we analyze the linguistic variation present across domains to identify key linguistic insights that can boost performance across domains. We propose methods to capture domain specific semantics of word usage in addition to global semantics. We then demonstrate how to effectively use such domain specific knowledge to learn NER models that outperform previous baselines in the domain adaptation setting.

==> definition.tex <==
\section{Problem Definition}
\todo{Merge above later}
We are given a series of corpora $\mathcal{C}=\{ C_{d_{1}}, C_{d_{2} } \dots C_{d_{k}} \}$ for which we would like to build Named Entity Recognition systems. Each $C_{d_{i}}$ corresponds to a different domain. In our setting labeled training data for these domains is scarce. Therefore trivially, training each model on its specific domain results in poor performance.  However we have access to a corpus $D$ for which we have significant amount of labeled training data.  We seek therefore to leverage this significant amount of labeled training data on $D$ to adapt and build models for each of the domains.

First, we build word representations (word embeddings) to effectively capture domain specific usage in an unsupervised fashion using large amounts of unlabeled data. We then use these domain specific embeddings to learn a NER model using supervised domain adaptation techniques \cite{jiang2008domain}.  Our NER model, which uses domain specific word embeddings outperforms previous methods and baselines on this task.  Finally, we also show apply our method in an active learning setting and demonstrate that by labeling only 2000 sentences in the target domain, we can achieve performance that is close to state of the art. 

In summary, we answer the following questions:
\begin{enumerate}[noitemsep, topsep=1pt]
\item Given a word $w$ how does its usage differ across different domains?
\item How can we effectively leverage these differences to build NER models that outperform baselines in the domain adaptation setting?
\end{enumerate}  
\label{sec:def}
